Pessimistic Backward Policy for GFlowNets

This paper studies Generative Flow Networks (GFlowNets), which learn to sample objects proportionally to a given reward function through the trajectory of state transitions. In this work, we observe that GFlowNets tend to under-exploit the high-reward objects due to training on insufficient number of trajectories, which may lead to a large gap between the estimated flow and the (known) reward value. In response to this challenge, we propose a pessimistic backward policy for GFlowNets (PBP-GFN), which maximizes the observed flow to align closely with the true reward for the object. We extensively evaluate PBP-GFN across eight benchmarks, including hyper-grid environment, bag generation, structured set generation, molecular generation, and four RNA sequence generation tasks. In particular, PBP-GFN enhances the discovery of high-reward objects, maintains the diversity of the objects, and consistently outperforms existing methods.

==> rebuttal.tex <==
\newpage

\input{resources/relative_mean_error}

\input{resources/fig_rebuttal_toy}

\input{resources/vs_reward_buffer_local_search}

.

\newpage

==> reproducibility.tex <==
\section{Reproducibility}

We conduct experiments on the official implementation of the referenced paper described in \Cref{appx:exp_setup} which also provides the detailed model architecture and hyper-parameters. 




==> resources/figure_highlevelmode.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.27\linewidth}
\centering
  \includegraphics[width=\linewidth]{iclr/resources/figures/VEM-L14-1_re_m.pdf}
  \subcaption{RNA-A}\label{subfig:RNA_A_mode2}
\end{subfigure}
\quad\;
\begin{subfigure}[t]{0.27\linewidth}
\centering
  \includegraphics[width=\linewidth]{iclr/resources/figures/VEM-L14-2_re_m.pdf}
  \caption{RNA-B}\label{subfig:RNA_B_mode2}
\end{subfigure}
\quad\;
\begin{subfigure}[t]{0.27\linewidth}
\centering
  \includegraphics[width=\linewidth]{iclr/resources/figures/VEM-L14-3_re_m.pdf}
  \subcaption{RNA-C}\label{subfig:RNA_C_mode2}
\end{subfigure}
\hfill
\caption{N-hamming ball}\label{fig:variance}
\vspace{-.15in}
\end{figure}


==> resources/figure_our.tex <==
\begin{figure}[t]
\centering
% \begin{subfigure}[t]{0.35\linewidth}
% \centering
  \includegraphics[width=\linewidth]{iclr/resources/figures/method.pdf}
% \end{subfigure}
\caption{\textbf{Pessimistic backward policy for GFlowNets (PBP-GFN).} The portion of the circle indicates the amount of flow. The black lines and the gray lines indicate the observed and unobserved trajectories, respectively. (\textbf{left}) Flow matching succeeds with the entire trajectories. (\textbf{middle}) Flow matching fails with partially observed trajectories. (\textbf{right}) PBP-GFN assigns high probabilities to the backward transitions of observed trajectories to keep a high probability to high-reward objects.
}\label{fig:method}
\end{figure}

==> resources/figure_qm9.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.3\linewidth}
\centering
  \includegraphics[width=0.9\linewidth]{example-image}
  \subcaption{Number of mode founds}\label{subfig:qm9_mode}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.3\linewidth}
\centering
  \includegraphics[width=0.9\linewidth]{example-image}
  \caption{Top-100 performance}\label{subfig:qm9_top100}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.3\linewidth}
\centering
  \includegraphics[width=0.9\linewidth]{example-image}
  \subcaption{Pearson correlation}\label{subfig:qm9_variance}
\end{subfigure}
\caption{QM9}\label{fig:qm9}
\end{figure}


==> resources/tab_acc.tex <==
\begin{table*}[t]
\centering
\caption{Accuracy.}\label{tab:reasoning}
\vspace{-.1in}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{Molecule} & \multicolumn{4}{c}{RNA sequence} \\
\cmidrule(lr){1-2}\cmidrule(lr){2-3}\cmidrule(lr){4-7}
Method & \multicolumn{1}{c}{sEH} & \multicolumn{1}{c}{QM9} & \multicolumn{1}{c}{TFBind8}  & \multicolumn{1}{c}{RNA-A} & \multicolumn{1}{c}{RNA-B} & \multicolumn{1}{c}{RNA-C} \\
\midrule
SoftQ \citep{xx} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
A2C \citep{xx} &  00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
\midrule
DB \citep{bengio2021gflownet} &  00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
SubTB \citep{madan2023learning} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
TB \citep{malkin2022trajectory} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
MaxEnt \citep{malkin2022trajectory} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
%SubGFN \citep{towardsunderstandinggflownets} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
GAFN \citep{pan2023generative} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
\midrule
FPB-GFN (ours) & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} & 00.0\stdv{0.0} \\
\bottomrule
\end{tabular}
}
\end{table*}

